Neural Face Rigging for Animating and Retargeting Facial Meshes in the Wild

We propose an end-to-end deep-learning approach for automatic rigging and retargeting of 3D models of human faces in the wild. Our approach, called Neural Face Rigging (NFR), holds three key properties: (i) NFR's expression space maintains human-interpretable editing parameters for artistic controls; (ii) NFR is readily applicable to arbitrary facial meshes with different connectivity and expressions; (iii) NFR can encode and produce fine-grained details of complex expressions performed by arbitrary subjects. To the best of our knowledge, NFR is the first approach to provide realistic and controllable deformations of in-the-wild facial meshes, without the manual creation of blendshapes or correspondence. We design a deformation autoencoder and train it through a multi-dataset training scheme, which benefits from the unique advantages of two data sources: a linear 3DMM with interpretable control parameters as in FACS, and 4D captures of real faces with fine-grained details. Through various experiments, we show NFR's ability to automatically produce realistic and accurate facial deformations across a wide range of existing datasets as well as noisy facial scans in-the-wild, while providing artist-controlled, editable parameters.

==> sec7_figsonly.tex <==
\newpage

\begin{figure*}
  \centering
    \includegraphics[width=0.5\linewidth]{figures/in-the-wild_new.jpg}
  \caption{
  \label{Fig:in-the-wild}
  \textbf{In-the-wild retargeting}. We apply NFR to transfer the expression of a facial mesh to another. \textcolor{myyellow}{Yellow}: target expression of  non-rigged face meshes with complex expressions composed of unknown AUs. 
  %The MetaHuman source is posed with its rig, then baked the deformation to the face mesh without the rig.
  \textcolor{cyan}{Cyan}: retargeted results of various face models. Note the robustness of NFR to the variations in identity, expression, triangulation, and mesh quality.}
\end{figure*}

\begin{figure}[H]
  \centering
    \includegraphics[width=\linewidth]{figures/sequence_editing_fig.jpg}
  \caption{
  \label{Fig:editing}
  \textbf{Human-friendly editing}. \textcolor{myyellow}{Yellow}:  non-rigged face mesh. Gray: Meshes after editing AUs.  Vertices are colored by the Euclidean distance before and after each modification.}
\end{figure}


% This big figure is placed in the end.
 \begin{figure*}[t]
  \centering
    \includegraphics[width=0.6\textwidth]{figures/blendshape_activation.jpg}
  \caption{\textbf{Disentangled latent code visualization.} We show the first 53 activations of our latent code on a \emph{MetaHuman} face. Each activation follows closely the pre-defined semantics of the FACS.}
  \label{fig:blendshape}
 \end{figure*}



\begin{figure}[H]
  \centering
    \includegraphics[width=\linewidth]{figures/non-linear-better.png}
  \caption{\textbf{Linear (top) vs. non-linear (bottom) models.} Simultaneous AU activation in linear models such as \emph{ICT FaceKit} ends up with unnatural deformations. The non-linearity in NFR helps ensure rational deformations.}
  \label{Fig:reasonable}
\end{figure}

\newpage

 \begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{ablation_ICT.png}
\caption{\textbf{Ablation showing the importance of synthetic data (\emph{ICT FaceKit}).} We show the effects of the first five AUs on \emph{Multiface} without training on \emph{ICT FaceKit}. The deformations are highly entangled and impractical for human editing.}
\label{Fig:ablation_ICT}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/data_argumentation_ab.jpg}
\caption{\textbf{Qualitative ablation of our data augmentation.} Without (\textbf{top}) vs. with (\textbf{bottom}) data augmentation. (a), (b) from \emph{FaceWarehouse} , (c), (d) from \emph{Triplegangers}. Our data augmentation is critical to NFR working on these in-the-wild meshes.}
\label{fig:argumentation-ab}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{figures/z_ablation.pdf}
\caption{\todo{Add an additional example}\textbf{Effect of $z_{ext}$.} Left: without the extended latent space, $z_{FACS}$ gets contaminated with entangled deformation in \emph{Multiface}. Right: with the extended latent space, $z_{FACS}$ successfully captures the disentangled deformation with correct semantics.}
\label{fig:z-extend-ab}
\end{figure}

\newpage



